What Drives the (In)stability of a Stablecoin?

In May 2022, an apparent speculative attack, followed by market panic, led to the precipitous downfall of UST, one of the most popular stablecoins at that time. However, UST is not the only stablecoin to have been depegged in the past. Designing resilient and long-term stable coins, therefore, appears to present a hard challenge. To further scrutinize existing stablecoin designs and ultimately lead to more robust systems, we need to understand where volatility emerges. Our work provides a game-theoretical model aiming to help identify why stablecoins suffer from a depeg. This game-theoretical model reveals that stablecoins have different price equilibria depending on the coin's architecture and mechanism to minimize volatility. Moreover, our theory is supported by extensive empirical data, spanning $1$ year. To that end, we collect daily prices for 22 stablecoins and on-chain data from five blockchains including the Ethereum and the Terra blockchain.

==> back.tex <==
\section{How stablecoins work}
\label{sec:back}

In this section, we discuss the peg defense mechanism of each of the four categorizations of stablecoin in more detail as well as provide real world examples of each categorizations. While all four types of stablecoin rely on the redemption against a reserve, they differs in the composition of the reserves and how redemption is conducted.

\subsection{Fiat-collateralized stablecoins}
Fiat-collateralized stablecoins are stablecoins that can be redeemed directly as a corresponding fiat currency. A major portion of their reserves is made of fiat or fiat-equivalent assets, such as short-dated U.S. treasury bills. Other portion of the reserves could consist of loans or even precious metals. Some examples of fiat-collateralized stablecoins are USDT, USDC, and USDP. The key distinctions of fiat-collateralized stablecoin are as followed: 1) Their reserves consist mainly of fiat or fiat-equivalent assets. 2) Minting or redeeming them are done with 1:1 ratio with fiat currencies in terms of value.

\subsection{Crypto-collateralized stablecoins}
Crypto-collateralized stablecoin is a term often associated with a broad categorization of any stablecoin that can be redeemed into cryptocurrencies. However, in this study, we further partition this broad categorization based on how redemption takes place. In this study, crypto-collateralized stablecoins refers to stablecoins that possess the following 3 characteristics. 1) Their reserves are composed of cryptocurrencies. 2) Redemption returns a basket of cryptocurrencies with approximately 1:1 in value of the redeemed stablecoins. 3) The stablecoin protocol has no control over expansion and contraction of the supply of the redeemed currencies; the redeemed currencies are not minted and burned during redemption and creation of the stablecoins, respectively. Given the volatility of cryptocurrency market, it is possible that the reserve of a crypto-collateralized stablecoin to be worth less than the supply of the it. To compensate for the higher risk of a bank-run event, crypto-collateralized stablecoin protocols often implement another peg defense mechanism. Those that use only crypto-collateralization as the only peg defense mechanism either have their reserves consist of only other stablecoins and relies on the reserves' price stability or have a way to accrue more value to their reserves. 

\subsection{Algorithmic stablecoins}
Similar to crypto-collateralized stablecoins, algorithmic stablecoins can be redeemed for cryptocurrencies. Unlike crypto-collateralized stablecoins, however, algorithmic stablecoin protocols have control over the expansion and contraction of their reserve currencies. Upon redemption, the reserve currencies are minted at 1:1 value ratio as the redeemed stablecoins. Given this, algorithmic stablecoins are characterized by the following 3 characteristics: 1) Redemption returns a basket of cryptocurrencies with approximately 1:1 in value of the redeemed stablecoins. 2) Redeemed cryptocurrencies are minted as opposed from being transferred from the reserve. 3) The stablecoin protocol has control over the expansion and contraction of supply of the redeemed currency. The expansion and contraction of supply of the redeemed token allows a flow of economic value between the stablecoin and redeemed token. USDT an example of an algorithmic stablecoin.

\subsection{Over-collateralized stablecoins} 
Over-collateralized stablecoins is another type of stablecoins that returns a basket of cryptocurrencies upon redemption. Issuance and redemption of over-collateralized stablecoins rely on a lending protocol backbone, where a basket of cryptocurrencies can be deposited into the reserve to issue stablecoins valuing less than the deposited collateral, hence 'over-collateralized'. Unlike crypto-collateralized stablecoins, the value held in their reserves are guaranteed to be greater than or equal to the stablecoin supply in normal working conditions. This property is derived from liquidation events in the lending protocol backbone if the value of the deposited basket of cryptocurrencies risk falling below the outstanding stablecoin debt. In this paper, we characterize over-collateralized stablecoins with the following characteristics: 1) Their reserves are composed of cryptocurrencies. 2) Redemption returns a basket of cryptocurrencies valued higher than the redeemed stablecoins. 3) There exists a liquidation mechanism ensuring that the value of the reserve is higher than the stablecoin supply. 4) The stablecoin protocol has no control over expansion and contraction of the supply of the redeemed currencies.
%Most recently, Terra, which was one of the most representative stablecoins, collapsed. 



==> intuition.tex <==
\vspace{-3mm}
\section{Intuition}
\vspace{-3mm}

%Here, we describe intuitions of the stablecoin model before diving into it. %We starts with a simple idea. 
%Traditionally, people have believed that users would be paid \$1 by the system when redeeming stablecoins. However, it may not be true depending on the asset type that the system uses to pay the users. 
%
While typical stablecoin systems rely on paying users the target price upon redemption, the payment that users realize can be lower depending on the reserve type.
%Fiat-collateralized systems use fiat money, whereas other types, such as crypto-collateralized, algorithmic, and over-collateralized systems use cryptocurrencies. 
%For example, consider cryptocurrencies employed in other types except fiat-collateralized systems. The price of a cryptocurrency constantly fluctuates. Even if a system pays users \$1 based on its price oracle, the actual payoff of users can be less than \$1 when a cryptocurrency depreciates, because the time difference between prices to which the system and users refer would exist due to non-zero transaction time, a discrete price oracle update within the system, etc. 
For example, consider stablecoin systems with cryptocurrency reserves. With the price volatility of the reserves, even if a system pays users \$1 based on its price oracle, the actual payoff of users can be less than \$1 when a cryptocurrency depreciates, because the time difference between prices to which the system and users refer would exist due to non-zero transaction time, a discrete price oracle update within the system, etc. 
Due to the user payoff of less than \$1, arbitrage between the stablecoin system and the secondary market would not operate even if the market price is less than \$1, which leads to the depeg.

The situation can deteriorate if a system uses weak assets to back its stablecoin. 
The system releases the assets backing the stablecoin on the market when purchasing stablecoins from users. Given this, users' redemption can decrease the price of the asset backing the stablecoin, and this influence would become greater when the asset value is largely derived from the system's usage. 
For example, recall the severe price drop of Luna due to the significant UST redemption of users in the second week of May, 2022. Back then, even though the system paid users \$1 based on its Luna price oracle, users would not actually have expected to earn \$1 by a rapid drop in Luna's price. Note that its value relies on the system's usage rather than external sources because it is an endogenous asset. 

% To escape from the depegging state, a system exploiting cryptocurrencies would need to pay more than \$1 to users when buying stablecoins from them, which makes their actual payoff not less than \$1. 
% Alternatively, it would be necessary to incentivize users to keep their stablecoins and not sell them in the market.  
%
With these intuitions in mind, we propose a game-theoretical model to quantify the risks of stablecoins.

==> related.tex <==
\section{Related Work}
\label{sec:related}
%\vspace{-3mm}

Models explaining the (in)stability of stablecoins are relatively sparse. \cite{klages2022while,klages2021stability} model stablecoins like Dai, where issuance is based on a market for leverage. In this context, they characterize deleveraging spirals that caused instability in Dai on `Black Thursday' in March 2020. \cite{lyons2020keeps} models how stablecoins backed by 100\% reserves, such as USDC, maintain stability through arbitrage with minting and redemption.

As discussed in \cite{klages2020stablecoins}, models of bank runs \cite{diamond1983bank}, runs on currency pegs \cite{morris1998unique}, and pegged redemption money market funds \cite{parlatore2016fragility} can be applied to understand many other types of stablecoins.
%bank run = assets may cover liabilities, but some assets are illiquid and not all stablecoins can be redeemed at one point in time (but may over time)
%run on currency peg = assets partially cover liabilities and not all stablecoins can be redeemed for peg value
%Pegged redemption money market funds face similar issues if net asset value falls below the pegged redemption rate.
\cite{routledge2022currency,li2020managing} discussed and created adaptations of these types of models specific to stablecoins.
These models can be applied to many types of decentralized stablecoins (e.g., algorithmic stablecoins), after reinterpreting the protocol as the central bank, as well as custodial stablecoins, and so basic results about bank and currency runs translate to many stablecoin settings.
In the context of these models, \cite{klagesmundt2022designing} characterize many stablecoins based on the shape of redemption curves and then design a redemption curve that attains properties informed by currency peg models.

Various distinctions about decentralized stablecoin models are not as developed, however, such as modeling the fact that reserve assets are not the currency target (e.g., USD is not an on-chain asset).
We address this by proposing a new game-theoretical model to include reserve assets that change in price and further by breaking down assets backing into exogenous and endogenous assets, which have different degrees of price risk.
In addition, there is room to expand a common model to better characterize nuanced differences across different types of stablecoins, which is the approach we take in analyzing redemption mechanisms in different stablecoins.
